Model Selection for Bayesian Autoencoders

We develop a novel method for carrying out model selection for Bayesian autoencoders (BAEs) by means of prior hyper-parameter optimization. Inspired by the common practice of type-II maximum likelihood optimization and its equivalence to Kullback-Leibler divergence minimization, we propose to optimize the distributional sliced-Wasserstein distance (DSWD) between the output of the autoencoder and the empirical data distribution. The advantages of this formulation are that we can estimate the DSWD based on samples and handle high-dimensional problems. We carry out posterior estimation of the BAE parameters via stochastic gradient Hamiltonian Monte Carlo and turn our BAE into a generative model by fitting a flexible Dirichlet mixture model in the latent space. Consequently, we obtain a powerful alternative to variational autoencoders, which are the preferred choice in modern applications of autoencoders for representation learning with uncertainty. We evaluate our approach qualitatively and quantitatively using a vast experimental campaign on a number of unsupervised learning tasks and show that, in small-data regimes where priors matter, our approach provides state-of-the-art results, outperforming multiple competitive baselines.

==> Makefile <==
# LaTeX setup
MAIN_TEX := main
TEX_ENGINE := pdflatex
LATEXMK := latexmk
BIBTEX_ENGINE := bibtex
TEX_FLAGS := -shell-escape
LATEXMK_FLAGS := -recorder -shell-escape -interaction=nonstopmode  -synctex=1 #-quiet
PDF_FILE := $(MAIN_TEX).pdf
TEX_COMMAND := $(TEX_ENGINE) $(TEX_FLAGS)

# Docker setup
PWD := $(shell pwd)
DOCKER_IMAGE := srossi/latex:2019
DOCKER_CONTAINER_NAME := latexmk-$(shell basename $(PWD))-$(MAIN_TEX)
DOCKER_RUN_DEAMON := docker run --rm -dt -v $(PWD):$(PWD) --workdir $(PWD) --name $(DOCKER_CONTAINER_NAME) --user="$(shell id -u):$(shell id -g)" $(DOCKER_IMAGE)
DOCKER_RUN := docker run --rm -it -v $(PWD):$(PWD) --workdir $(PWD) --user="$(shell id -u):$(shell id -g)" $(DOCKER_IMAGE)
DOCKER_IT := docker run --rm -it -v $(PWD):$(PWD) --workdir $(PWD)  $(DOCKER_IMAGE)

TEX_FILES := $(shell find . -type f -name "*.tex")
BIB_FILES := $(shell find . -type f -name "*.bib")
TIKZ_FILES := $(shell find . -type f -name "*.tikz")
 
#	Set up viewer and number of parallel jobs for figures
VIEWER :=
UNAME_S := $(shell uname -s)
ifeq ($(UNAME_S),Linux)
    VIEWER = okular
    NJOBS=$(shell nproc --all)
endif
ifeq ($(UNAME_S),Darwin)
    VIEWER = open -a Skim
    NJOBS=$(shell sysctl -n hw.ncpu)
endif

#	Set up latexmk flags
ifeq ($(TEX_ENGINE),pdflatex)
	LATEXMK_FLAGS += -pdf
else
	LATEXMK_FLAGS += -$(TEX_ENGINE)
endif

# -include $(MAIN_TEX).makefile

pdf: $(PDF_FILE)

docker:
	@$(DOCKER_RUN) $(LATEXMK) $(LATEXMK_FLAGS) -quiet -g $(MAIN_TEX) 


$(PDF_FILE): $(TEX_FILES) $(BIB_FILES) $(TIZK_FILES)
	latexmk $(LATEXMK_FLAGS) -quiet -g $(MAIN_TEX) 


deamon-start:
	@$(DOCKER_RUN_DEAMON) $(LATEXMK) $(LATEXMK_FLAGS) -quiet -pvc -g $(MAIN_TEX) 

deamon-attach: 
	@docker container attach $(DOCKER_CONTAINER_NAME)

deamon-stop:
	@docker container stop $(DOCKER_CONTAINER_NAME)

interactive:
	@$(DOCKER_IT) 

indent:
	@$(DOCKER_RUN)  find . -type f -name "*tex"  -exec latexindent --overwrite -s {} \;

view: 
	$(VIEWER) $(PDF_FILE) &

clean:
	@rm -rf *.sav *.bak *.aux *.bcf *.fdb_latexmk *acn *glo *ist *.fls *.makefile *.run.xml *.bbl *.blg *.figlist *.log  *.out *.toc *.xdv *auxlock *dvi *lof *lol *lot thesis-blx.bib *tdo *acr *alg *dvi *glg *gls *mw *synctex* *.pdf
	find . -name "*.log" -type f -delete
	find . -name "*.dep" -type f -delete
	find . -name "*.dpth" -type f -delete
	find . -name "*.aux" -type f -delete
	find . -name "*bak*" -type f -delete
	find . -name "*.glo*" -type f -delete
	find . -name "*.ist*" -type f -delete
	find . -name "*.acn*" -type f -delete

	
superclean: clean
	@find figures -name "*.pdf" -type f -delete
	@find figures -name "*.md5" -type f -delete


